Further results on Minimal and Minimum Cylindrical Algebraic Decompositions

We consider cylindrical algebraic decompositions (CADs) as a tool for representing semi-algebraic subsets of $\mathbb{R}^n$. In this framework, a CAD $\mathscr{C}$ is adapted to a given set $S$ if $S$ is a union of cells of $\mathscr{C}$. Different algorithms computing an adapted CAD may produce different outputs, usually with redundant cell divisions. In this paper we analyse the possibility to remove the superfluous data. We thus consider the set $\text{CAD}^r(\mathcal{F})$ of CADs of class $C^r$ ($r \in \mathbb{N} \cup \{\infty, \omega\}$) that are adapted to a finite family $\mathcal{F}$ of semi-algebraic sets of $\mathbb{R}^n$, endowed with the refinement partial order and we study the existence of minimal and minimum element in $\text{CAD}^r(\mathcal{F})$. We show that for every such $\mathcal{F}$ and every $\mathscr{C} \in \text{CAD}^r(\mathcal{F})$, there is a minimal CAD of class $C^r$ adapted to $\mathcal{F}$ and smaller (i.e. coarser) than or equal to $\mathscr{C}$. In dimension $n=1$ or $n=2$, this result is strengthened by proving the existence of a minimum element in $\text{CAD}^r(\mathcal{F})$. In contrast, for any $n \geq 3$, we provide explicit examples of semi-algebraic sets whose associated poset of adapted CADs does not admit a minimum. We then introduce a reduction relation on $\text{CAD}^r(\mathcal{F})$ in order to define an algorithm for the computation of minimal CADs and we characterise those semi-algebraic sets $\mathcal{F}$ for which $\text{CAD}^r(\mathcal{F})$ has a minimum by means of confluence of the associated reduction system. We finally provide practical criteria for deciding if a semi-algebraic set does admit a minimum CAD and apply them to describe various concrete examples of semi-algebraic sets, along with their minimum CAD of class $C^r$.

==> topology-test.tex <==
\section{Topology induced by a CAD}

We denote by $\mathcal{T}_{\text{eucl}}$ the euclidean topology on $\R^n$.
\begin{definition}
    Let $\Cr$ be a CAD of $\R^n$. 
    \begin{enumerate}
        \item For all cell $C \in \Cr$, we write $\mathcal{T}_C$ the topology on $C$ induced by $\mathcal{T}_{\text{eucl}}$. 
        \item The topology $\mathcal{T}_{\Cr}$ on $\R^n$  associated with $\Cr$ is defined as the topology whose basic open sets are $\bigcup \{\mathcal{T}_C \; | \; C \in \Cr\}.$
        \item The collection of all topologies associated with a $\CAD^r$ adapted to $\Fr$ is $\mathbb{T}(\CAD^r(\Fr))$.
    \end{enumerate}
\end{definition}

\begin{lemma}
    The connected components of $(\R^{n}, \mathcal{T}_{\Cr})$ are exactly the cells of $\Cr$.
\end{lemma}
\begin{proof}
    \red{todo}
\end{proof}
\begin{proposition}
    Let $\Cr$ and $\Cr'$ be two CADs. We have $\Cr \preceq \Cr'$ if and only if $\mathcal{T}_{\Cr} \subseteq \mathcal{T}_{\Cr'}$. In particular, The poset $(\CAD^0(\Fr), \preceq)$ admits a minimum if and only if the poset $(\mathbb{T}(\CAD^0(\Fr)), \subseteq)$ admits a minimum.
\end{proposition}
\begin{proof}
    \red{todo}
\end{proof}

% \begin{corollary}
%     The poset $(\CAD^0(\Fr), \preceq)$ admits a minimum if and only if the poset $(\mathbb{T}(\CAD^0(\Fr)), \subseteq)$ admits a minimum.
% \end{corollary}
% \begin{proof}
%     Evident vu la prop précédente.
% \end{proof}


\begin{definition}\mbox{}
\begin{enumerate}
    \item For every $\mathfrak{b} \in \mathfrak{B}$ of length $2l+1$ and every $x \in B(\Fr, \mathfrak{b})$, we write $$\cup_{i=1}^p \partial (S_i)_x = \{f^1_{\mathfrak{b}}(x), \ldots, f^l_{\mathfrak{b}}(x)\}$$ with $f^i_{\mathfrak{b}}(x) < f^j_{\mathfrak{b}}(x)$ when $1 \leq i < j \leq l$.

    \item We denote by $\mathcal{T}^{\Fr}_{\mathfrak{b}}$ the initial topology on $B(\Fr, \mathfrak{b})$ with respect to the family
    $$\{f^1_{\mathfrak{b}}, \ldots, f^l_{\mathfrak{b}} : B(\Fr, \mathfrak{b}) \to (\R, \mathcal{T}_\text{eucl})\}$$ 
    where $\R^l$ is endowed with the euclidean topology. 

    \item The topology $\mathcal{T}^{\Fr}_{\mathfrak{B}}$ on $\R^{n-1}$ associated with the behaviours of $\Fr$ is defined as the topology whose basic open sets are $\bigcup \{\mathcal{T}^{\Fr}_{ \mathfrak{b}} \; | \; \mathfrak{b} \in \mathfrak{B}\}.$
\end{enumerate}
\end{definition}

% \begin{remark}
%     For every $\mathfrak{b} \in \mathfrak{B}$, the topology $\mathcal{T}^{\Fr}_{\mathfrak{b}}$ coincide with the initial topology with respect to the map 
%     $$B(\Fr, \mathfrak{b}) \to (\R^l,\mathcal{T}_{\text{eucl}})  : x \mapsto \cup \; \partial \Fr_x.$$
%     \blue{Ca n'apporte rien.}
% \end{remark}
\begin{proposition}
    Let $\Dr$ be a CAD of $\R^{n-1}$. We have $\Dr \in \pi_{n-1}(\CAD^r(\Fr))$ if and only if $\mathcal{T}^{\Fr}_{\mathfrak{B}} \subseteq \mathcal{T}_{\Dr}.$
\end{proposition}
\begin{proof}
    \red{todo}
\end{proof}

\begin{example}
    Denote by $X$ the line of equation $y = 0 \land z = 0$. Take the overapproximation $\mathcal{O} = \{\Dr \in \CAD^r(\R^{n-1}) \; | \; X \in \mathcal{T}_{\Dr}\}$ to show that the two semi-algebraic sets depicted below have a minimum CAD.

            \begin{figure}[H]
    \center
    %\includegraphics[scale=0.35]{figures/2parabolas3D.png}
      \includegraphics[scale=0.25]{figures/parchemin-v1.png} \; \;
        \includegraphics[scale=0.25]{figures/parchemin-v2.png}
    \caption{Parchemins}
    \label{fig:last}
\end{figure}
\end{example}
